VasoMIM: Vascular Anatomy-Aware Masked Image Modeling for Vessel Segmentation

Accurate vessel segmentation in X-ray angiograms is crucial for numerous clinical applications. However, the scarcity of annotated data presents a significant challenge, which has driven the adoption of self-supervised learning (SSL) methods such as masked image modeling (MIM) to leverage large-scale unlabeled data for learning transferable representations. Unfortunately, conventional MIM often fails to capture vascular anatomy because of the severe class imbalance between vessel and background pixels, leading to weak vascular representations. To address this, we introduce Vascular anatomy-aware Masked Image Modeling (VasoMIM), a novel MIM framework tailored for X-ray angiograms that explicitly integrates anatomical knowledge into the pre-training process. Specifically, it comprises two complementary components: anatomy-guided masking strategy and anatomical consistency loss. The former preferentially masks vessel-containing patches to focus the model on reconstructing vessel-relevant regions. The latter enforces consistency in vascular semantics between the original and reconstructed images, thereby improving the discriminability of vascular representations. Empirically, VasoMIM achieves state-of-the-art performance across three datasets. These findings highlight its potential to facilitate X-ray angiogram analysis.

==> Fig_Vessel_Patch_Ratio_Epoch.tex <==
\begin{figure}[htbp]
	\centerline{\includegraphics{figs/fig_vessel_patch_epoch_ratio.pdf}}
	\caption{Proportion of vessel-containing patches in the masked patches of each epoch.}
	\label{fig:vessel_patch_ratio_epoch}
\end{figure}

==> Fig_Vessel_Patch_Ratio_Vis.tex <==
\begin{figure}[htbp]
	\centerline{\includegraphics{figs/fig_vessel_patch_ratio_vis.pdf}}
	\caption{Patch-wise masking ratio during the pre-training process.}
	\label{fig:vessel_patch_ratio_vis}
\end{figure}

==> Section0_Checklist.tex <==
Unless specified otherwise, please answer ``yes'' to each question if the relevant information is described either in the paper itself or in a technical appendix with an explicit reference from the main paper. If you wish to explain an answer further, please do so in a section titled ``Reproducibility Checklist'' at the end of the technical appendix.

\noindent This paper:
\begin{itemize}
    \item Includes a conceptual outline and/or pseudocode description of AI methods introduced (yes/partial/no/NA) \\
    \textbf{Answer}: yes
    
    \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results (yes/no) \\
    \textbf{Answer}: yes

    \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper (yes/no) \\
    \textbf{Answer}: yes
\end{itemize}

\noindent Does this paper make theoretical contributions? (yes/no)

\textbf{Answer}: no

\noindent If yes, please complete the list below.
\begin{itemize}
    \item All assumptions and restrictions are stated clearly and formally. (yes/partial/no)
    \item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)
    \item Proofs of all novel claims are included. (yes/partial/no)
    \item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)
    \item Appropriate citations to theoretical tools used are given. (yes/partial/no)
    \item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)
    \item All experimental code used to eliminate or disprove claims is included. (yes/no/NA)
\end{itemize}

\noindent Does this paper rely on one or more datasets? (yes/no)

\textbf{Answer}: yes

\noindent If yes, please complete the list below.
\begin{itemize}
    \item A motivation is given for why the experiments are conducted on the selected datasets (yes/partial/no/NA) \\
    \textbf{Answer}: yes

    \item All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA) \\
    \textbf{Answer}: yes

    \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA) \\
    \textbf{Answer}: partial
    
    \item All datasets drawn from the existing literature (potentially including authors' own previously published work) are accompanied by appropriate citations. (yes/no/NA) \\
    \textbf{Answer}: yes

    \item All datasets drawn from the existing literature (potentially including authors' own previously published work) are publicly available. (yes/partial/no/NA) \\
    \textbf{Answer}: partial

    \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/NA) \\
    \textbf{Answer}: yes
\end{itemize}

\noindent Does this paper include computational experiments? (yes/no)

\textbf{Answer}: yes

\noindent If yes, please complete the list below.
\begin{itemize}
    \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA) \\
    \textbf{Answer}: yes

    \item Any code required for pre-processing data is included in the appendix. (yes/partial/no) \\
    \textbf{Answer}: yes

    \item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no) \\
    \textbf{Answer}: yes

    \item All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no) \\
    \textbf{Answer}: yes

    \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes/partial/no) \\
    \textbf{Answer}: yes

    \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA) \\
    \textbf{Answer}: yes

    \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no) \\
    \textbf{Answer}: partial

    \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no) \\
    \textbf{Answer}: yes

    \item This paper states the number of algorithm runs used to compute each reported result. (yes/no) \\
    \textbf{Answer}: yes

    \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no) \\
    \textbf{Answer}: yes

    \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no) \\
    \textbf{Answer}: no

    \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper's experiments. (yes/partial/no/NA). \\
    \textbf{Answer}: yes
\end{itemize}

==> Table_S2W.tex <==
\begin{table}[htbp]
\centering
\renewcommand\arraystretch{1.2}
\begin{tabular}{lllll}
\toprule
\multirow{2}{*}{Manner} & \multirow{2}{*}{$\beta_0$} & \multirow{2}{*}{$\beta_E$} & \multicolumn{2}{c}{DSC (\%)} \\ \cmidrule{4-5} 
 & & & ARCADE & CAXF \\ \midrule
 Random & $0$ & $0$ & $68.45$ & $84.03$ \\
 \cellcolor{gray!20}Weak-to-Strong & \cellcolor{gray!20}$0$ & \cellcolor{gray!20}$0.5$ & \cellcolor{gray!20}$\mathbf{68.85}$ & \cellcolor{gray!20}$\mathbf{84.49}$ \\
 \multicolumn{1}{l}{Strong-to-Weak} & \multicolumn{1}{l}{$0.5$} & \multicolumn{1}{l}{$0$} & \multicolumn{1}{l}{$67.81$} & \multicolumn{1}{l}{$83.41$} \\
 \bottomrule
\end{tabular}
\caption{Comparison of weak-to-strong and strong-to-weak anatomical guidance. DSC is reported in this table.}
\label{table:s2w}
\end{table}
